Comparative Analysis of Transfer Learning in Deep Learning Text-to-Speech Models on a Few-Shot, Low-Resource, Customized Dataset

Text-to-Speech (TTS) synthesis using deep learning relies on voice quality. Modern TTS models are advanced, but they need large amount of data. Given the growing computational complexity of these models and the scarcity of large, high-quality datasets, this research focuses on transfer learning, especially on few-shot, low-resource, and customized datasets. In this research, "low-resource" specifically refers to situations where there are limited amounts of training data, such as a small number of audio recordings and corresponding transcriptions for a particular language or dialect. This thesis, is rooted in the pressing need to find TTS models that require less training time, fewer data samples, yet yield high-quality voice output. The research evaluates TTS state-of-the-art model transfer learning capabilities through a thorough technical analysis. It then conducts a hands-on experimental analysis to compare models' performance in a constrained dataset. This study investigates the efficacy of modern TTS systems with transfer learning on specialized datasets and a model that balances training efficiency and synthesis quality. Initial hypotheses suggest that transfer learning could significantly improve TTS models' performance on compact datasets, and an optimal model may exist for such unique conditions. This thesis predicts a rise in transfer learning in TTS as data scarcity increases. In the future, custom TTS applications will favour models optimized for specific datasets over generic, data-intensive ones.

==> literature_review.tex <==
\chapter{Literature Review}




\section{Advancements in Spectrogram-Based Text-to-Speech Synthesis}

Text-to-speech (TTS) synthesis has undergone significant evolution, with a predominant focus on spectrogram-based models that harness the prowess of neural architectures to drive improvements in voice cloning and generate expressive, natural speech. Starting with foundational works like Tacotron (Wang et al.) and its sequel, Tacotron 2 (Shen et al.), the landscape saw the introduction of end-to-end models adept at converting text into mel-scale spectrograms which could then be translated to audio waveforms. While these models have garnered accolades for their mean opinion scores (MOS) in comparison to traditional TTS systems, their autoregressive nature has been a point of contention due to relatively slow inference times for lengthier sequences.

Addressing such concerns, the emergence of Glow-TTS (Kim et al.) and SpeedySpeech (Vainer and Dušek) was notable. Glow-TTS integrated flow-based generative paradigms with a knack for learning autonomous alignment, which in turn could predict non-overlapping output frames at each decoding instance. This design innovation, coupling flows with dynamic programming, slashed inference times dramatically, enhancing its viability for on-the-fly applications. SpeedySpeech, a derivative of the student-teacher architecture, similarly delivered high-quality audio synthesis at remarkable speeds, notably by sidelining the dependency on self-attention layers.

Yet, the drive for innovation didn't stop there. AlignTTS by Zeng et al. introduced a novel feed-forward architecture, focusing on parallel TTS synthesis. Its ingenuity lies in a specially crafted alignment loss inspired by the revered Baum-Walch algorithm. As a result, AlignTTS surpassed Transformer TTS models, yet at a speed that was over 50 times faster. In another intriguing development, FastPitch (Ła\'ncucki) brought pitch prediction into the spotlight during the inference phase, lending a touch of emotion and expressiveness to the resultant speech.

In the more recent spectrum, SC-GlowTTS (Casanova et al., 2023) has emerged as a force to reckon with, especially in scenarios with speakers not seen during the training phase. Here, the flow-based model is augmented with a speaker-conditional blueprint, aiming for zero-shot multi-speaker TTS synthesis. The integration of a GAN-based vocoder further elevates the similarity and quality of speech, even for newly-introduced speakers.

Further enriching the corpus of research, Battenberg et al. (2023) with Capacitron and Mehta et al. (2023) through their OverFlow model and subsequent works, have dived deep into the intricacies of TTS latent variable models, variational embedding, and the fusion of traditional and contemporary TTS paradigms. These works underscore the potential of probabilistic modeling, flow-based techniques, and variational embeddings in enhancing TTS synthesis.

In summation, the extensive advancements in spectrogram-based TTS models underscore a vibrant journey from the foundational Tacotron systems to the contemporary works of SC-GlowTTS and OverFlow. The consistent endeavor has been to elevate speech quality, reduce inference times, and enhance voice similarity, especially with unseen speakers. As this domain continues to mature, we remain hopeful for groundbreaking innovations that further refine voice cloning, especially in multilingual contexts, thus bridging linguistic divides seamlessly.


\section{Exploration of Attention Methods in Text-to-Speech Systems}

End-to-end text-to-speech (TTS) systems, primarily dominated by recurrent neural networks, have been effective in transforming the landscape of speech synthesis. However, their requirement of considerable computational resources and extended training times are persistent challenges. Recent research efforts have begun focusing on attention methods, exploring alternative architectures and regularization techniques that alleviate these issues and improve the quality and naturalness of speech synthesis.

A significant milestone in this domain was the development of the Deep Convolutional TTS (DCTTS) proposed by Hideyuki Tachibana, Katsuya Uenoyama, and Shunsuke Aihara. Unlike conventional TTS systems, DCTTS was based entirely on deep convolutional neural networks (CNNs), eliminating the use of recurrent units. This design change resulted in a substantial reduction in training times, with an ordinary gaming PC achieving satisfactory results overnight. Although the system's architecture mirrored that of Tacotron, a salient feature of DCTTS was the introduction of a 'guided attention' mechanism, contributing to efficient attention module training. This work represented a significant stride in reducing the economic costs of TTS system training.

In a similar vein, Yibin Zheng and his team tackled the issue of exposure bias in TTS systems. They proposed two methods aimed at harmonizing the sequences predicted by forward and backward decoding. The first method introduced divergence regularization terms into the model training objective, reducing the disagreement between left-to-right (L2R) and right-to-left (R2L) directional models. The second method centered on decoder-level improvements, utilizing future information during decoding and implementing a joint training strategy. These innovations demonstrated marked improvements in system robustness and overall naturalness, outperforming the baseline Tacotron2 model and nearing human quality in mean opinion score (MOS) tests.

Complementing these strides, Eric Battenberg and his team proposed two new families of attention mechanisms - location-relative Gaussian Mixture Model (GMM)-based mechanisms and additive energy-based mechanisms. These were designed to tackle the prevalent issue of text alignment failures in attention-based TTS systems. The researchers introduced enhancements to GMM-based attention for rapid and consistent alignment during training. Furthermore, they introduced the Dynamic Convolution Attention (DCA) mechanism, a purely location-based mechanism that excelled in generalizing to very long utterances. The results demonstrated that both GMM attention and DCA maintained naturalness for shorter utterances while improving robustness significantly for longer ones.

In summary, the literature presents a substantial body of work focusing on alternative architectures and attention mechanisms for TTS systems. These efforts strive to reduce training times, improve speech quality, and enhance the overall robustness of TTS systems. While advancements have been significant, continual research and development are expected to further the field and provide ever more efficient and effective solutions in voice synthesis and voice cloning.


\section{Vocoder}
Vocoders, which are pivotal in modern text-to-speech and audio synthesis systems, have seen significant advances, particularly with the application of Generative Adversarial Networks (GANs). Key improvements have centered on waveform generation speed, audio quality, and model efficiency.

Kundan Kumar et al. [1] introduced MelGAN, a Generative Adversarial Network model for conditional waveform synthesis. This non-autoregressive, feed-forward, fully convolutional architecture was a significant step forward in raw audio generation with GANs, with a notable ten-fold increase in generation speed compared to previous models. It was demonstrated to be a suitable replacement for autoregressive models in various applications, despite slight quality degradation.

Building on the MelGAN architecture, Geng Yang et al. [2] proposed Multi-band MelGAN (MB-MelGAN), which significantly reduced the computational complexity of the original model and enhanced its speed. The use of a multi-resolution STFT loss and an increase in the receptive field of the generator were significant contributors to these improvements, leading to high mean opinion scores (MOS) in waveform generation and text-to-speech applications.

Ryuichi Yamamoto et al. [3] introduced the Parallel WaveGAN, an effective parallel waveform generation model. By employing a joint optimization method between the adversarial loss and multi-resolution short-time Fourier transform (STFT) loss, it improved the time-frequency distributions of the realistic speech signal. This model significantly outpaced conventional ClariNet models and matched their quality, using a fraction of the parameters.

In another exploration, Bi\'nkowski et al. [4] proposed GAN-TTS, a Generative Adversarial Network for Text-to-Speech with an ensemble of discriminators and a feed-forward generator. The model demonstrated that adversarially trained feed-forward generators can indeed synthesize high-fidelity speech audio. Its novel application of Fréchet Inception Distance (FID) and Kernel Inception Distance (KID) metrics for speech generation contributed to the model's effectiveness.

Chen et al. [5] introduced WaveGrad, a model that combines techniques from score matching and diffusion probabilistic models for waveform generation. Notably, WaveGrad offers an inherent trade-off between inference speed and sample quality by adjusting the number of refinement steps. This approach narrows the gap between non-autoregressive and autoregressive models in terms of audio quality.

HiFi-GAN, presented by Kong et al. [6], achieved both efficient and high-fidelity speech synthesis. This model utilized a novel multi-period discriminator, which consisted of multiple sub-discriminators each handling a portion of periodic signals of input audio. It outperformed state-of-the-art models like WaveNet and WaveGlow in terms of audio quality and generation speed.

Finally, Won Jang et al. [7] introduced UnivNet, which employed a multi-resolution spectrogram discriminator to synthesize high-fidelity waveforms in real-time. Its impressive performance on both seen and unseen speakers showed its adaptability and effectiveness, and it outperformed other GAN-based vocoders in objective and subjective evaluations.

In conclusion, these studies have made substantial strides in the domain of vocoders, exploiting GAN architectures to enhance waveform generation speed, improve audio quality, and minimize computational complexity. Current efforts are directed towards resolving the trade-off between speed and audio quality, maximizing model efficiency, and improving the adaptability of these models to unseen speakers.



\section{End-to-end models}
The field of voice cloning and text-to-speech (TTS) synthesis has seen significant advancements in recent years, with a focus on end-to-end models that can generate natural-sounding speech in the voice of different speakers, including those unseen during training.

One such model is the SV2TTS proposed by Ye Jia et al., which consists of three independently trained components: a speaker encoder network, a sequence-to-sequence synthesis network based on Tacotron 2, and an auto-regressive WaveNet-based vocoder network. The speaker encoder network is trained on a speaker verification task using an independent dataset of noisy speech without transcripts from thousands of speakers. The system is able to synthesize natural speech from speakers unseen during training, with the quality of the synthesized speech improving when the speaker encoder is trained on a large and diverse speaker set [1].

Jaehyeon Kim, Jungil Kong, and Juhee Son proposed a parallel end-to-end TTS method that generates more natural-sounding audio than current two-stage models. Their model adopts variational inference augmented with normalizing flows and an adversarial training process, which improves the expressive power of generative modeling. They also propose a stochastic duration predictor to synthesize speech with diverse rhythms from input text [2].

Edresson Casanova et al. presented YourTTS, a multilingual approach to the task of zero-shot multi-speaker TTS. YourTTS builds upon the VITS model and adds several novel modifications for zero-shot multi-speaker and multilingual training. The model uses raw text as input instead of phonemes, allowing more realistic results for languages without good open-source grapheme-to-phoneme converters available [3].

James Betker presents TorToise, an expressive, multi-voice TTS system that applies advances in the image generative domain to speech synthesis. The system combines autoregressive decoders and denoising diffusion probabilistic models (DDPMs), which have demonstrated the ability to scale performance with additional compute and data [4].

Eugene Kharitonov et al. introduced SPEAR-TTS, a multi-speaker TTS system that can be trained with minimal supervision. SPEAR-TTS combines two types of discrete speech representations to cast TTS as a composition of two sequence-to-sequence tasks: from text to high-level semantic tokens (akin to "reading") and from semantic tokens to low-level acoustic tokens ("speaking"). Decoupling these two tasks enables training of the "speaking" module using abundant audio-only data, and unlocks the highly efficient combination of pre-training and backtranslation to reduce the need for parallel data when training the "reading" component [5].

These studies demonstrate the potential of end-to-end models for voice cloning and TTS synthesis, and provide a foundation for the development of more advanced systems that can generate high-quality, natural-sounding speech in a variety of voices and languages.

\section{Advancements in Spoken Language Processing: A Review of Recent Studies}
Recent years have seen an increased interest in the development of spoken language processing tools and techniques. The studies presented in this literature review have shed light on advancements in this field and the wide variety of tasks that these models can handle, such as automatic speech recognition, speech synthesis, speech translation, voice conversion, speech enhancement, and speaker identification.

In the study by Changhan Wang et al. (2021), they introduced the FAIRSEQ S2 extension to FAIRSEQ, a toolkit developed for scalable and integrable speech synthesis. This toolkit includes several autoregressive and non-autoregressive text-to-speech models and offers several benefits, such as scalability and easy integration with other systems. Furthermore, it includes a suite of automatic metrics that speed up development and analysis and implements preprocessing tools to facilitate the training of speech synthesis models with less curated data. The FAIRSEQ S2 has demonstrated superior performance across various spoken language processing tasks.

Advancing on the same theme, Junyi Ao et al. (2022) proposed a unified-modal SpeechT5 framework that utilizes an encoder-decoder pre-training for self-supervised speech/text representation learning. This model includes a shared encoder-decoder network and six modal-specific pre/post-nets. The SpeechT5 model demonstrated its superiority over a wide variety of spoken language processing tasks.

In a more specific context, Chengyi Wang et al. proposed VALL-E, a language modeling approach for text-to-speech synthesis (TTS) that leverages large, diverse, and multi-speaker speech data. Unlike conventional approaches, VALL-E uses discrete codes derived from an off-the-shelf neural audio codec model and approaches TTS as a conditional language modeling task. It was found to significantly outperform the state-of-the-art zero-shot TTS system in terms of speech naturalness and speaker similarity. Interestingly, VALL-E can synthesize high-quality personalized speech with just a 3-second recording from an unseen speaker, indicating its promising potential in practical applications.

In a further development, Ziqiang Zhang et al. (2023) extended the concept of VALL-E to VALL-E X for cross-lingual speech synthesis. This model presents an attractive solution for challenges in cross-lingual speech synthesis, such as data scarcity and model capacity. It shows high capability in terms of preserving the speaker's voice, emotion, and acoustic environment and effectively addresses the foreign accent issues. VALL-E X opens up new avenues for applications such as zero-shot cross-lingual text-to-speech synthesis and zero-shot speech-to-speech translation tasks.

Finally, a team from Meta AI embarked on an ambitious project known as the Massively Multilingual Speech (MMS) project, aiming to drastically expand the language coverage of speech technology. They created pre-trained wav2vec 2.0 models covering over 1,000 languages, a single multilingual automatic speech recognition model, speech synthesis models, and a language identification model. They used a new dataset based on readings of publicly available religious texts and leveraged self-supervised learning. This project not only brings speech technology to more people but also contributes to the preservation of linguistic diversity worldwide.

In summary, these studies present cutting-edge techniques and methods that advance our understanding and application of spoken language processing. They reveal the effectiveness of self-supervised learning, large-scale diverse data, and innovative approaches in dealing with various tasks in this field. Future research may build upon these findings to further refine these models and explore their potential in practical applications.



